Image Classification in the Dark using Quanta Image Sensors

State-of-the-art image classifiers are trained and tested using well-illuminated images. These images are typically captured by CMOS image sensors with at least tens of photons per pixel. However, in dark environments when the photon flux is low, image classification becomes difficult because the measured signal is suppressed by noise. In this paper, we present a new low-light image classification solution using Quanta Image Sensors (QIS). QIS are a new type of image sensors that possess photon counting ability without compromising on pixel size and spatial resolution. Numerous studies over the past decade have demonstrated the feasibility of QIS for low-light imaging, but their usage for image classification has not been studied. This paper fills the gap by presenting a student-teacher learning scheme which allows us to classify the noisy QIS raw data. We show that with student-teacher learning, we are able to achieve image classification at a photon level of one photon per pixel or lower. Experimental results verify the effectiveness of the proposed method compared to existing solutions.

==> TeX/customFigureMacros.tex <==
% ===========================================================
% Definitions, commands and environnments for drawing figures
%
% Vivek Goyal
% based on work by
% Ivana Jovanovic, Patrick Vandewalle, Olivier Roy - 2005
% ===========================================================

% --------
% PACKAGES
% --------
%\RequirePackage{amsmath}
%\RequirePackage{amssymb}
\RequirePackage{xspace}
\RequirePackage{bbm}
\RequirePackage{ifthen}
%\RequirePackage{pstricks}
%\RequirePackage{pst-plot}
%\RequirePackage{algo}
%\RequirePackage{epsfig}
%\RequirePackage{latexsym}
%\RequirePackage{subfigure}

% --------------------
% PSTRICKS DEFINITIONS
% --------------------
% Upsampling operation (reference point at the center of the circle)
% Parameter #1: upsampling factor
\def\upsampling#1{

    \pscircle(0,0){0.5}
    \psline{->}(-0.15,-0.25)(-0.15,0.25)
    \rput(0.15,0){#1}

}

% Downsampling operation (reference point at the center of the circle)
% Parameter #1: downsampling factor
\def\downsampling#1{

    \pscircle(0,0){0.5}
    \psline{<-}(-0.15,-0.25)(-0.15,0.25)
    \rput(0.15,0){#1}

}

% Sampling operation (reference point at the center of the box)
% Parameter #1: sampling period
% This is a quick-and-dirty job; definitely less beautiful than other macros.
\def\sampler#1{

    \psframe(-1,-0.5)(1,0.5)
    \psline{-}(-0.6,-0.2)(-0.2,-0.2)
    \psline{-}(0.2,-0.2)(0.6,-0.2)
    \psline{-}(-0.2,-0.2)(0.1,0.1)
    \rput(-0.3,0.3){#1}

}

% Discrete-to-continuous operation (reference point at the center of the box)
% (Generation of weighted Dirac train)
% Parameter #1: sampling period
% This is a quick-and-dirty job; definitely less beautiful than other macros.
\def\diracTrain#1{

    \psframe(-1,-0.5)(1,0.5)
    \psline{-}(-0.8,0)(0.8,0)
    \psline{->}(-0.6,0)(-0.6,-0.45)
    \psline{->}(-0.3,0)(-0.3,-0.3)
    \psline{->}( 0.0,0)( 0.0, 0.4)
    \psline{->}( 0.3,0)( 0.3, 0.4)
    \psline{->}( 0.6,0)( 0.6,-0.35)
    \rput(0.3,-0.2){#1}

}

% Filter (reference point at the center of the box)
% Parameter #1: filter label
\def\filter#1{

    \psframe(-1,-0.5)(1,0.5)
    \rput(0,0){#1}

}

\def\shortfilter#1{

    \psframe(-0.75,-0.5)(0.75,0.5)
    \rput(0,0){#1}

}

% Filter (reference point at the center of the box)
% Parameter #1: filter label
\def\widefilter#1{

    \psframe(-2,-0.5)(2,0.5)
    \rput(0,0){#1}

}

% Sum (reference point at the center of the circle)
\def\sumsymbol{

    \pscircle(0,0){0.25}
    \rput(0,0){$+$}

}

% Analysis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: downsampling factor
\def\analysis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\downsampling{#2}}
    \psline{-}(4,0)(4.5,0)
}

% Analysis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: downsampling factor
\def\wideanalysis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(2.5,0){\widefilter{#1}}
    \psline{-}(4.5,0)(5,0)
    \rput(5.5,0){\downsampling{#2}}
    \psline{-}(6,0)(6.5,0)
}

% Synthesis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: synthesis filter label
% Parameter #2: upsampling factor
\def\synthesis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(2,0)
    \rput(3,0){\filter{#1}}
    \psline{-}(4,0)(4.5,0)
}

% Filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: synthesis filter label
% Parameter #3: down/upsampling factor
\def\filterbankchannel#1#2#3{

    \rput(0,0){\analysis{#1}{#3}}
    \rput(4.5,0){\synthesis{#2}{#3}}

}

% Two channel filter bank (reference point at the begining of the filter bank)
% Parameter #1: lowpass analysis filter label
% Parameter #2: lowpass synthesis filter label
% Parameter #3: highpass analysis filter label
% Parameter #4: highpass synthesis filter label

\def\twochannelfilterbank#1#2#3#4{

    % Input
    \psline{*-}(0,0)(0.5,0)
    \psline{-}(0.5,-0.75)(0.5,0.75)

    % Highpass branch
    \rput(0.5,0.75){\filterbankbranch{#3}{#4}{2}}

    % Lowpass branch
    \rput(0.5,-0.75){\filterbankbranch{#1}{#2}{2}}

    % Output
    \psline{->}(9.5,0.75)(9.5,0.25)
    \rput(9.5,0){\sumsymbol}
    \psline{->}(9.5,-0.75)(9.5,-0.25)
    \psline{-*}(9.75,0)(10.25,0)

}




% Parameter #1: filter label
% Parameter #2: sampling factor
% Parameter #3: delay
\def\mybranch#1#2#3{
    \psline{-}(0,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(2,0)
    \rput(2.75,0){\shortfilter{#3}}
    \psline{-}(3.5,0)(4,0)
    \rput(5,0){\filter{#1}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8,0)
}


\def\mybranchA#1#2{
    \psline{-}(-0.5,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(4,0)
    \rput(5,0){\filter{#1}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8.5,0)
}


\def\mybranchB#1#2#3{
    \psline{-}(0,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\upsampling{#2}}
    \psline{-}(4,0)(4.5,0)
    \rput(5.25,0){\shortfilter{#3}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8,0)
}


\def\mybranchC#1#2{
    \psline{-}(-0.5,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\upsampling{#2}}
    \psline{-}(4,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8.5,0)
}
